CountingDINO: A Training-free Pipeline for Class-Agnostic Counting using Unsupervised Backbones

Class-agnostic counting (CAC) aims to estimate the number of objects in images without being restricted to predefined categories. However, while current exemplar-based CAC methods offer flexibility at inference time, they still rely heavily on labeled data for training, which limits scalability and generalization to many downstream use cases. In this paper, we introduce CountingDINO, the first training-free exemplar-based CAC framework that exploits a fully unsupervised feature extractor. Specifically, our approach employs self-supervised vision-only backbones to extract object-aware features, and it eliminates the need for annotated data throughout the entire proposed pipeline. At inference time, we extract latent object prototypes via ROI-Align from DINO features and use them as convolutional kernels to generate similarity maps. These are then transformed into density maps through a simple yet effective normalization scheme. We evaluate our approach on the FSC-147 benchmark, where we consistently outperform a baseline based on an SOTA unsupervised object detector under the same label- and training-free setting. Additionally, we achieve competitive results -- and in some cases surpass -- training-free methods that rely on supervised backbones, non-training-free unsupervised methods, as well as several fully supervised SOTA approaches. This demonstrates that label- and training-free CAC can be both scalable and effective. Code: https://lorebianchi98.github.io/CountingDINO/.

==> sec/CARPK_qualitatives/old/XX_qualitativesCARPK_0.tex <==

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\figimg}[1]{\includegraphics[width=\figw, height=2.5cm]{#1}}
\arrayrulecolor{gray}

\begin{figure*}[h]
    \centering
    \tiny
    \newcommand{\hd}[1]{\textbf{#1}}
    \newcommand{\figw}{.26\textwidth}
    \setlength{\tabcolsep}{1pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{*6{C{\figw}}} %\begin{tabular}{r>{\hspace{0.1cm}}*6{p{\figw}>{\hspace{2pt}}}}

        \midrule % Row 1
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00272.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00251.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00140.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00228.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00431.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00281.png} \\
        \rowcolor[gray]{.9}
        146 &
        155 &
        130 &
        54 &
        142 &
        139 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00272.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00272.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00251.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00251.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00140.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00140.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00228.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00228.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00431.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00431.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00281.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00281.png} 
 \\
        81.9 &
        81.0 &
        161.0 &
        52.9 &
        152.4 &
        94.6 \\

        \midrule % Row 2
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00290.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00316.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00046.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00349.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00211.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00249.png} \\
        \rowcolor[gray]{.9}
        139 &
        82 &
        141 &
        117 &
        23 &
        154 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00290.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00290.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00316.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00316.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00046.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00046.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00349.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00349.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00211.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00211.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00249.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00249.png} 
 \\
        93.2 &
        90.5 &
        180.6 &
        82.3 &
        34.6 &
        105.7 \\

        \midrule % Row 3
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00040.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00026.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00245.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00299.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00101.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00003.png} \\
        \rowcolor[gray]{.9}
        113 &
        107 &
        118 &
        75 &
        97 &
        67 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00040.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00040.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00026.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00026.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00245.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00245.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00299.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00299.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00101.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00101.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00003.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00003.png} 
 \\
        131.1 &
        170.1 &
        71.7 &
        70.3 &
        103.8 &
        67.8 \\


    \midrule
    \end{tabular}
    }
    \caption{\textbf{Qualitative results.}}
    \label{fig:more-examples-0}
\end{figure*}


==> sec/CARPK_qualitatives/old/XX_qualitativesCARPK_1.tex <==

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\figimg}[1]{\includegraphics[width=\figw, height=2.5cm]{#1}}
\arrayrulecolor{gray}

\begin{figure*}[h]
    \centering
    \tiny
    \newcommand{\hd}[1]{\textbf{#1}}
    \newcommand{\figw}{.26\textwidth}
    \setlength{\tabcolsep}{1pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{*6{C{\figw}}} %\begin{tabular}{r>{\hspace{0.1cm}}*6{p{\figw}>{\hspace{2pt}}}}

        \midrule % Row 4
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00280.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00252.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00086.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00038.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00064.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00275.png} \\
        \rowcolor[gray]{.9}
        134 &
        152 &
        112 &
        108 &
        110 &
        141 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00280.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00280.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00252.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00252.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00086.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00086.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00038.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00038.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00064.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00064.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00275.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00275.png} 
 \\
        71.8 &
        100.1 &
        219.1 &
        118.6 &
        135.2 &
        100.3 \\

        \midrule % Row 5
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00037.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00111.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00269.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00180.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00354.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00325.png} \\
        \rowcolor[gray]{.9}
        103 &
        73 &
        155 &
        116 &
        129 &
        122 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00037.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00037.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00111.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00111.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00269.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00269.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00180.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00180.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00354.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00354.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00325.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00325.png} 
 \\
        114.2 &
        93.7 &
        93.3 &
        141.1 &
        118.9 &
        135.6 \\

        \midrule % Row 6
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00418.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00224.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00109.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00066.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00134.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00201.png} \\
        \rowcolor[gray]{.9}
        148 &
        52 &
        74 &
        120 &
        117 &
        6 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00418.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00418.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00224.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00224.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00109.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00109.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00066.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00066.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00134.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00134.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00201.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00201.png} 
 \\
        218.3 &
        56.0 &
        86.1 &
        138.5 &
        200.6 &
        8.2 \\

        \midrule % Row 7
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00217.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00069.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00361.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00210.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00240.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00265.png} \\
        \rowcolor[gray]{.9}
        42 &
        118 &
        119 &
        21 &
        124 &
        156 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00217.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00217.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00069.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00069.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00361.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00361.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00210.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00210.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00240.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00240.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00265.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00265.png} 
 \\
        52.8 &
        175.8 &
        118.1 &
        86.1 &
        61.0 &
        107.8 \\

        \midrule % Row 8
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00031.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00089.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00108.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00401.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00193.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00052.png} \\
        \rowcolor[gray]{.9}
        103 &
        116 &
        73 &
        50 &
        37 &
        126 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00031.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00031.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00089.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00089.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00108.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00108.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00401.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00401.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00193.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00193.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00052.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00052.png} 
 \\
        124.6 &
        124.7 &
        86.3 &
        57.8 &
        41.5 &
        203.8 \\

        \midrule % Row 9
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00320.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00149.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00146.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00318.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00411.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00029.png} \\
        \rowcolor[gray]{.9}
        80 &
        112 &
        118 &
        80 &
        137 &
        104 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00320.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00320.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00149.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00149.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00146.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00146.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00318.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00318.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00411.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00411.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00029.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00029.png} 
 \\
        89.6 &
        113.5 &
        207.4 &
        144.2 &
        98.2 &
        197.5 \\


    \midrule
    \end{tabular}
    }
    \caption{\textbf{Qualitative results.}}
    \label{fig:more-examples-1}
\end{figure*}


==> sec/CARPK_qualitatives/old/XX_qualitativesCARPK_2.tex <==

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\figimg}[1]{\includegraphics[width=\figw, height=2.5cm]{#1}}
\arrayrulecolor{gray}

\begin{figure*}[h]
    \centering
    \tiny
    \newcommand{\hd}[1]{\textbf{#1}}
    \newcommand{\figw}{.26\textwidth}
    \setlength{\tabcolsep}{1pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{*6{C{\figw}}} %\begin{tabular}{r>{\hspace{0.1cm}}*6{p{\figw}>{\hspace{2pt}}}}

        \midrule % Row 10
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00028.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00023.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00115.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00058.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00050.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00012.png} \\
        \rowcolor[gray]{.9}
        99 &
        106 &
        73 &
        116 &
        141 &
        103 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00028.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00028.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00023.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00023.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00115.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00115.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00058.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00058.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00050.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00050.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00012.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00012.png} 
 \\
        126.6 &
        188.9 &
        67.9 &
        129.8 &
        131.9 &
        112.0 \\

        \midrule % Row 11
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00135.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00241.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00429.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00203.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00124.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00237.png} \\
        \rowcolor[gray]{.9}
        122 &
        125 &
        165 &
        6 &
        81 &
        109 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00135.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00135.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00241.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00241.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00429.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00429.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00203.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00203.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00124.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00124.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00237.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00237.png} 
 \\
        218.0 &
        75.6 &
        126.8 &
        10.7 &
        89.6 &
        63.6 \\

        \midrule % Row 12
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00337.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00400.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00442.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00301.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00288.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00285.png} \\
        \rowcolor[gray]{.9}
        132 &
        39 &
        161 &
        81 &
        142 &
        142 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00337.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00337.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00400.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00400.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00442.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00442.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00301.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00301.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00288.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00288.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00285.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00285.png} 
 \\
        102.4 &
        43.6 &
        117.9 &
        196.8 &
        88.9 &
        146.1 \\

        \midrule % Row 13
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00407.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00239.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00313.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00178.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00165.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00215.png} \\
        \rowcolor[gray]{.9}
        110 &
        138 &
        74 &
        117 &
        111 &
        34 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00407.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00407.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00239.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00239.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00313.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00313.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00178.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00178.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00165.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00165.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00215.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00215.png} 
 \\
        119.0 &
        74.8 &
        81.4 &
        176.5 &
        118.3 &
        40.6 \\

        \midrule % Row 14
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00092.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00372.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00051.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00005.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00347.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00091.png} \\
        \rowcolor[gray]{.9}
        117 &
        115 &
        139 &
        80 &
        129 &
        117 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00092.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00092.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00372.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00372.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00051.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00051.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00005.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00005.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00347.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00347.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00091.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00091.png} 
 \\
        145.7 &
        108.1 &
        231.4 &
        79.7 &
        91.7 &
        217.9 \\

        \midrule % Row 15
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00397.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00230.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00119.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00061.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00399.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00250.png} \\
        \rowcolor[gray]{.9}
        13 &
        58 &
        73 &
        111 &
        30 &
        157 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00397.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00397.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00230.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00230.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00119.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00119.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00061.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00061.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00399.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00399.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00250.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00250.png} 
 \\
        10.9 &
        130.6 &
        78.4 &
        186.2 &
        79.5 &
        94.9 \\


    \midrule
    \end{tabular}
    }
    \caption{\textbf{Qualitative results.}}
    \label{fig:more-examples-2}
\end{figure*}


==> sec/CARPK_qualitatives/old/XX_qualitativesCARPK_3.tex <==

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\figimg}[1]{\includegraphics[width=\figw, height=2.5cm]{#1}}
\arrayrulecolor{gray}

\begin{figure*}[h]
    \centering
    \tiny
    \newcommand{\hd}[1]{\textbf{#1}}
    \newcommand{\figw}{.26\textwidth}
    \setlength{\tabcolsep}{1pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{*6{C{\figw}}} %\begin{tabular}{r>{\hspace{0.1cm}}*6{p{\figw}>{\hspace{2pt}}}}

        \midrule % Row 16
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00267.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00198.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00292.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00256.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00345.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00125.png} \\
        \rowcolor[gray]{.9}
        155 &
        4 &
        125 &
        146 &
        163 &
        90 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00267.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00267.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00198.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00198.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00292.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00292.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00256.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00256.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00345.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00345.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00125.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00125.png} 
 \\
        98.4 &
        6.8 &
        73.3 &
        88.8 &
        154.3 &
        104.2 \\

        \midrule % Row 17
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00072.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00437.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00013.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00167.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00261.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00386.png} \\
        \rowcolor[gray]{.9}
        115 &
        126 &
        104 &
        126 &
        143 &
        21 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00072.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00072.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00437.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00437.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00013.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00013.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00167.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00167.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00261.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00261.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00386.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00386.png} 
 \\
        152.8 &
        125.4 &
        108.5 &
        141.1 &
        97.0 &
        15.7 \\

        \midrule % Row 18
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00427.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00276.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00209.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00117.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00080.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00384.png} \\
        \rowcolor[gray]{.9}
        163 &
        142 &
        19 &
        73 &
        110 &
        39 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00427.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00427.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00276.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00276.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00209.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00209.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00117.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00117.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00080.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00080.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00384.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00384.png} 
 \\
        86.4 &
        72.4 &
        28.5 &
        82.7 &
        117.6 &
        47.8 \\

        \midrule % Row 19
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00335.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00412.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00382.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00187.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00408.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00331.png} \\
        \rowcolor[gray]{.9}
        173 &
        138 &
        51 &
        109 &
        123 &
        188 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00335.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00335.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00412.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00412.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00382.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00382.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00187.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00187.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00408.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00408.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00331.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00331.png} 
 \\
        384.9 &
        135.6 &
        47.3 &
        126.3 &
        83.4 &
        130.5 \\

        \midrule % Row 20
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00247.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00370.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00059.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00104.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00085.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00202.png} \\
        \rowcolor[gray]{.9}
        149 &
        116 &
        118 &
        81 &
        110 &
        6 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00247.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00247.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00370.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00370.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00059.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00059.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00104.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00104.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00085.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00085.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00202.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00202.png} 
 \\
        106.7 &
        112.8 &
        148.1 &
        130.5 &
        219.6 &
        11.3 \\

        \midrule % Row 21
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00340.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00036.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00279.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00396.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00284.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00041.png} \\
        \rowcolor[gray]{.9}
        140 &
        99 &
        135 &
        6 &
        144 &
        118 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00340.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00340.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00036.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00036.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00279.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00279.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00396.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00396.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00284.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00284.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00041.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00041.png} 
 \\
        93.0 &
        156.2 &
        64.1 &
        10.6 &
        88.0 &
        231.8 \\


    \midrule
    \end{tabular}
    }
    \caption{\textbf{Qualitative results.}}
    \label{fig:more-examples-3}
\end{figure*}


==> sec/CARPK_qualitatives/old/XX_qualitativesCARPK_4.tex <==

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\figimg}[1]{\includegraphics[width=\figw, height=2.5cm]{#1}}
\arrayrulecolor{gray}

\begin{figure*}[h]
    \centering
    \tiny
    \newcommand{\hd}[1]{\textbf{#1}}
    \newcommand{\figw}{.26\textwidth}
    \setlength{\tabcolsep}{1pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{*6{C{\figw}}} %\begin{tabular}{r>{\hspace{0.1cm}}*6{p{\figw}>{\hspace{2pt}}}}

        \midrule % Row 22
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00362.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00234.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00264.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00338.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00274.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00206.png} \\
        \rowcolor[gray]{.9}
        118 &
        76 &
        154 &
        133 &
        143 &
        9 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00362.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00362.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00234.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00234.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00264.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00264.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00338.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00338.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00274.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00274.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00206.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00206.png} 
 \\
        90.4 &
        68.0 &
        105.6 &
        102.5 &
        70.7 &
        12.1 \\

        \midrule % Row 23
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00017.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00055.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00025.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00268.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00182.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00404.png} \\
        \rowcolor[gray]{.9}
        112 &
        122 &
        108 &
        156 &
        111 &
        76 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00017.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00017.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00055.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00055.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00025.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00025.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00268.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00268.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00182.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00182.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00404.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00404.png} 
 \\
        186.1 &
        152.5 &
        114.3 &
        362.8 &
        130.0 &
        141.1 \\

        \midrule % Row 24
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00073.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00238.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00415.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00160.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00077.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00094.png} \\
        \rowcolor[gray]{.9}
        115 &
        124 &
        167 &
        114 &
        111 &
        106 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00073.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00073.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00238.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00238.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00415.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00415.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00160.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00160.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00077.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00077.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00094.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00094.png} 
 \\
        178.0 &
        80.6 &
        228.4 &
        147.9 &
        193.5 &
        127.1 \\

        \midrule % Row 25
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00030.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00093.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00054.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00253.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00170.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00283.png} \\
        \rowcolor[gray]{.9}
        101 &
        111 &
        121 &
        151 &
        119 &
        142 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00030.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00030.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00093.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00093.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00054.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00054.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00253.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00253.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00170.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00170.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00283.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00283.png} 
 \\
        188.9 &
        121.0 &
        124.2 &
        72.3 &
        216.5 &
        94.0 \\

        \midrule % Row 26
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00456.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00430.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00332.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00196.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00414.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00151.png} \\
        \rowcolor[gray]{.9}
        73 &
        152 &
        186 &
        17 &
        144 &
        118 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00456.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00456.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00430.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00430.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00332.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00332.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00196.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00196.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00414.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00414.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00151.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00151.png} 
 \\
        80.4 &
        119.4 &
        199.6 &
        19.8 &
        254.5 &
        122.8 \\

        \midrule % Row 27
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00324.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00205.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00212.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00259.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00067.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00344.png} \\
        \rowcolor[gray]{.9}
        109 &
        8 &
        25 &
        142 &
        121 &
        156 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00324.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00324.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00205.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00205.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00212.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00212.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00259.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00259.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00067.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00067.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00344.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00344.png} 
 \\
        128.3 &
        12.5 &
        37.9 &
        87.6 &
        133.1 &
        187.2 \\


    \midrule
    \end{tabular}
    }
    \caption{\textbf{Qualitative results.}}
    \label{fig:more-examples-4}
\end{figure*}


==> sec/CARPK_qualitatives/old/XX_qualitativesCARPK_5.tex <==

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\figimg}[1]{\includegraphics[width=\figw, height=2.5cm]{#1}}
\arrayrulecolor{gray}

\begin{figure*}[h]
    \centering
    \tiny
    \newcommand{\hd}[1]{\textbf{#1}}
    \newcommand{\figw}{.26\textwidth}
    \setlength{\tabcolsep}{1pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{*6{C{\figw}}} %\begin{tabular}{r>{\hspace{0.1cm}}*6{p{\figw}>{\hspace{2pt}}}}

        \midrule % Row 28
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00254.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00434.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00441.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00039.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00194.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00070.png} \\
        \rowcolor[gray]{.9}
        145 &
        119 &
        161 &
        110 &
        24 &
        118 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00254.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00254.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00434.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00434.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00441.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00441.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00039.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00039.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00194.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00194.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00070.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00070.png} 
 \\
        240.4 &
        96.6 &
        85.7 &
        163.6 &
        26.9 &
        127.5 \\

        \midrule % Row 29
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00363.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00034.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00266.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00199.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00311.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00417.png} \\
        \rowcolor[gray]{.9}
        117 &
        91 &
        154 &
        4 &
        75 &
        140 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00363.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00363.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00034.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00034.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00266.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00266.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00199.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00199.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00311.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00311.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00417.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00417.png} 
 \\
        132.2 &
        99.4 &
        108.6 &
        18.1 &
        84.2 &
        88.7 \\

        \midrule % Row 30
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00262.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00263.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00138.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00001.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00391.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00355.png} \\
        \rowcolor[gray]{.9}
        149 &
        153 &
        114 &
        67 &
        2 &
        141 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00262.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00262.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00263.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00263.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00138.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00138.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00001.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00001.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00391.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00391.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00355.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00355.png} 
 \\
        95.1 &
        152.8 &
        128.2 &
        66.7 &
        29.4 &
        119.0 \\

        \midrule % Row 31
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00062.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00131.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00383.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00452.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00289.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00248.png} \\
        \rowcolor[gray]{.9}
        108 &
        108 &
        45 &
        97 &
        140 &
        150 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00062.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00062.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00131.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00131.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00383.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00383.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00452.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00452.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00289.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00289.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00248.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00248.png} 
 \\
        122.8 &
        199.1 &
        37.8 &
        116.2 &
        94.6 &
        98.9 \\

        \midrule % Row 32
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00303.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00204.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00282.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00398.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00200.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00063.png} \\
        \rowcolor[gray]{.9}
        85 &
        7 &
        138 &
        21 &
        6 &
        110 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00303.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00303.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00204.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00204.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00282.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00282.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00398.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00398.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00200.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00200.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00063.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00063.png} 
 \\
        56.7 &
        12.7 &
        82.6 &
        25.3 &
        13.3 &
        166.1 \\

        \midrule % Row 33
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00043.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00184.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00334.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00277.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00049.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00121.png} \\
        \rowcolor[gray]{.9}
        129 &
        106 &
        182 &
        139 &
        139 &
        73 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00043.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00043.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00184.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00184.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00334.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00334.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00277.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00277.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00049.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00049.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00121.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00121.png} 
 \\
        179.1 &
        185.3 &
        470.6 &
        87.4 &
        155.0 &
        76.8 \\


    \midrule
    \end{tabular}
    }
    \caption{\textbf{Qualitative results.}}
    \label{fig:more-examples-5}
\end{figure*}


==> sec/CARPK_qualitatives/old/XX_qualitativesCARPK_6.tex <==

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\figimg}[1]{\includegraphics[width=\figw, height=2.5cm]{#1}}
\arrayrulecolor{gray}

\begin{figure*}[h]
    \centering
    \tiny
    \newcommand{\hd}[1]{\textbf{#1}}
    \newcommand{\figw}{.26\textwidth}
    \setlength{\tabcolsep}{1pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{*6{C{\figw}}} %\begin{tabular}{r>{\hspace{0.1cm}}*6{p{\figw}>{\hspace{2pt}}}}

        \midrule % Row 34
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00183.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00380.png} \\
        \rowcolor[gray]{.9}
        112 &
        54 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00183.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00183.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00380.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00380.png} 
 \\
        146.0 &
        50.2 \\


    \midrule
    \end{tabular}
    }
    \caption{\textbf{Qualitative results.}}
    \label{fig:more-examples-6}
\end{figure*}


==> sec/CARPK_qualitatives/qualitativesCARPK_bad_0.tex <==

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
%\newcommand{\figimg}[1]{\includegraphics[width=\figw, height=2.5cm]{#1}}
\arrayrulecolor{gray}

\begin{figure*}[t]
    \centering
    \tiny
    \newcommand{\hd}[1]{\textbf{#1}}
    \newcommand{\figw}{.26\textwidth}
    \setlength{\tabcolsep}{1pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{*6{C{\figw}}} %\begin{tabular}{r>{\hspace{0.1cm}}*6{p{\figw}>{\hspace{2pt}}}}

        \midrule % Row 1
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00255.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00141.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00261.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00258.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00403.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00247.png} \\
        \rowcolor[gray]{.9}
        144 &
        138 &
        143 &
        142 &
        66 &
        149 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00255.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00255.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00141.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00141.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00261.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00261.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00258.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00258.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00403.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00403.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00247.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00247.png} 
 \\
        63.6 &
        199.7 &
        77.2 &
        61.8 &
        97.5 &
        60.6 \\

        \midrule % Row 2
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00333.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00046.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00253.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00287.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00284.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00180.png} \\
        \rowcolor[gray]{.9}
        183 &
        141 &
        151 &
        145 &
        144 &
        116 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00333.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00333.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00046.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00046.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00253.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00253.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00287.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00287.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00284.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00284.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00180.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00180.png} 
 \\
        124.7 &
        132.9 &
        80.6 &
        66.1 &
        88.1 &
        124.1 \\

        \midrule % Row 3
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00273.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00278.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00421.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00281.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00274.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00173.png} \\
        \rowcolor[gray]{.9}
        148 &
        137 &
        149 &
        139 &
        143 &
        119 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00273.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00273.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00278.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00278.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00421.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00421.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00281.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00281.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00274.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00274.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00173.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00173.png} 
 \\
        85.5 &
        71.2 &
        135.8 &
        77.9 &
        63.0 &
        244.0 \\


    \midrule
    \end{tabular}
    }
    \caption{\textbf{Qualitative results.}}
    \label{fig:more-examples-0}
\end{figure*}


==> sec/CARPK_qualitatives/qualitativesCARPK_bad_1.tex <==

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
%\newcommand{\figimg}[1]{\includegraphics[width=\figw, height=2.5cm]{#1}}
\arrayrulecolor{gray}

\begin{figure*}[t]
    \centering
    \tiny
    \newcommand{\hd}[1]{\textbf{#1}}
    \newcommand{\figw}{.26\textwidth}
    \setlength{\tabcolsep}{1pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{*6{C{\figw}}} %\begin{tabular}{r>{\hspace{0.1cm}}*6{p{\figw}>{\hspace{2pt}}}}

        \midrule % Row 4
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00211.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00277.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00266.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00259.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00416.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00331.png} \\
        \rowcolor[gray]{.9}
        23 &
        139 &
        154 &
        142 &
        139 &
        188 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00211.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00211.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00277.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00277.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00266.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00266.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00259.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00259.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00416.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00416.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00331.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00331.png} 
 \\
        30.7 &
        69.6 &
        81.1 &
        77.0 &
        187.4 &
        117.7 \\

        \midrule % Row 5
        \large
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00257.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00275.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00276.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00061.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00238.png} &
        \figimg{images/supplementary/CARPK/images/20161225_TPZ_00332.png} \\
        \rowcolor[gray]{.9}
        146 &
        141 &
        142 &
        111 &
        124 &
        186 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00257.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00257.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00275.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00275.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00276.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00276.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00061.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00061.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00238.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00238.png} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps_no_bkg_threshold/20161225_TPZ_00332.png}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/CARPK/densitymaps/20161225_TPZ_00332.png} 
 \\
        67.1 &
        66.4 &
        91.0 &
        180.7 &
        83.5 &
        116.0 \\


    \midrule
    \end{tabular}
    }
    \caption{\textbf{Qualitative results.}}
    \label{fig:more-examples-1}
\end{figure*}


==> sec/XX_CARPK_results.tex <==
\section{Quantitative Results on CARPK}

\begin{table*}[ht!]
\centering
\small
\begin{adjustbox}{width=\textwidth}
\begin{tabularx}{\textwidth}{l *{4}{>{\centering\arraybackslash}X}}
    \toprule
     &  \multicolumn{2}{c}{\textbf{Train}} & \multicolumn{2}{c}{\textbf{Test}} \\
    \cmidrule(r){2-3} \cmidrule(r){4-5}
      & MAE $\downarrow$ & RMSE $\downarrow$ & MAE $\downarrow$ & RMSE $\downarrow$ \\
    \toprule
    \rowcolor{lightgray}
    \multicolumn{5}{l}{\textit{A) Effect of Ellipse assumption}}  \\
    % without ellipse assumption
    w/o ellipse & \textbf{12.66} & \textbf{17.54} & 39.78 & 50.17 \\
    %DINO ViT B/8 & 23.25 & 32.21 & 53.58 & 61.52 \\
    %DINOv2 L/14 reg. & 12.66 & 17.54 & 39.78 & 50.17 \\
    %with ellipse
    w/ ellipse & 19.34 & 28.43 & \textbf{30.39} & \textbf{48.96} \\
    %DINO ViT B/8 & 43.29 & 61.69 & 42.23 & 59.36 \\
    %DINOv2 L/14 reg. & \textbf{19.34} & \textbf{28.43} & \textbf{30.39} & \textbf{48.96} \\
    \midrule
    \rowcolor{lightgray}
    \multicolumn{5}{l}{\textit{B) Effect of thresholding}}  \\
    %without threshold:
    w/o thresholding & 79.1 & 84.88 & 90.5 & 104.74 \\
    %DINO ViT B/8 & 105.27 & 114.61 & 101.58 & 117.92 \\
    %DINOv2 L/14 reg. & 79.1 & 84.88 & 90.5 & 104.74 \\
    %with threshold:
    w/ thresholding & \textbf{19.34} & \textbf{28.43} & \textbf{30.39} & \textbf{48.96} \\
    %DINO ViT B/8 & 43.29 & 61.69 & 42.23 & 59.36 \\
%DINOv2 L/14 reg. & \textbf{19.34} & \textbf{28.43} & \textbf{30.39} & \textbf{48.96} \\
    \midrule
    \rowcolor{lightgray}
    \multicolumn{5}{l}{\textit{D) Effect of changing the resolution}}  \\
    %resolution 1x
    Resolution 1x & \textbf{14.18} & \textbf{20.86} & 29.67 & \textbf{39.06} \\
    %DINO ViT B/8 & 13.04 & 16.96 & 38.88 & 46.64 \\
    %DINOv2 L/14 reg. & 14.18 & 20.86 & 29.67 & 39.06 \\
    %resolution 2x
    Resolution 2x & 14.56 & 22.49 & \textbf{27.38} & 40.16 \\
    %DINO ViT B/8 & 17.02 & 25.83 & 32.6 & 41.41 \\
    %DINOv2 L/14 reg. & 14.56 & 22.49 & 27.38 & 40.16 \\
    %resolution 4x
    Resolution 4x & 19.34 & 28.43 & 30.39 & 48.96 \\
    %DINO ViT B/8 & 43.29 & 61.69 & 42.23 & 59.36 \\
    %DINOv2 L/14 reg. & \textbf{19.34} & \textbf{28.43} & \textbf{30.39} & \textbf{48.96} \\
    \midrule
    \rowcolor{lightgray}
    \multicolumn{5}{l}{\textit{D) Effect of changing the backbone}}  \\
CLIP B/16 & 133.98 & 149.77 & 157.04 & 178.62 \\
CLIP L/14 & 120.81 & 142.62 & 131.36 & 155.96 \\
\hdashline
MAE B/16 & 112.47 & 128.08 & 146.86 & 170.48 \\
MAE L/16 & 129.09 & 142.19 & 159.01 & 182.23 \\
\hdashline
DINO ResNet50 & 64.84 & 78.07 & 81.72 & 103.26 \\
DINO ViT S/8 & 142.04 & 160.92 & 102.04 & 142.06 \\
DINO ViT B/8 & 43.29 & 61.69 & 42.23 & 59.36 \\
\hdashline
DINOv2 S/14 & 19.18 & 26.88 & 27.73 & 40.68 \\
DINOv2 B/14 & 16.58 & 24.07 & \textbf{25.99} & \textbf{38.42} \\
DINOv2 L/14 & \textbf{15.51} & \textbf{23.38} & 27.3 & 43.22 \\
DINOv2 S/14 reg. & 18.02 & 24.84 & 29.23 & 45.88 \\
DINOv2 B/14 reg. & 23.63 & 32.9 & 30.8 & 46.81 \\
DINOv2 L/14 reg. & 19.34 & 28.43 & 30.39 & 48.96 \\
\bottomrule
    \end{tabularx}
\end{adjustbox}
    \caption{\textbf{Ablation study on CARPK.} Impact of various components in our method. %: Sections \textit{A–C} assess individual processing choices, \textit{D} compares visual backbones, and \textit{E} evaluates the effect of exemplar count. 
    Unless specified otherwise, experiments use the DINOv2 ViT L/14 backbone with registers.}

    \label{tab:carpk_ablation}
\end{table*}



\begin{table*}[ht!]
\centering
\small
\begin{adjustbox}{width=\textwidth}
\begin{tabularx}{\textwidth}{l *{4}{>{\centering\arraybackslash}X}}
    \toprule
     &  \multicolumn{2}{c}{\textbf{Train}} & \multicolumn{2}{c}{\textbf{Test}} \\
    \cmidrule(r){2-3} \cmidrule(r){4-5}
      & MAE $\downarrow$ & RMSE $\downarrow$ & MAE $\downarrow$ & RMSE $\downarrow$ \\
    \toprule
    \rowcolor{lightgray}
    \multicolumn{5}{l}{\textit{A) Effect of Ellipse assumption}}  \\
    % without ellipse assumption
    w/o ellipse & \textbf{13.13} & \textbf{17.6} & 41.61 & 50.0 \\
    %DINOv2 B/14 & 13.13 & 17.6 & 41.61 & 50.0 \\
    %DINOv2 L/14 & 12.49 & 16.69 & 39.93 & 49.03 \\
    %with ellipse
    w/ ellipse & 16.58 & 24.07 & \textbf{25.99} & \textbf{38.42} \\
    %DINOv2 B/14 & 16.58 & 24.07 & \textbf{25.99} & \textbf{38.42} \\
    %DINOv2 L/14 & \textbf{15.51} & \textbf{23.38} & 27.3 & 43.22 \\
    \midrule
    \rowcolor{lightgray}
    \multicolumn{5}{l}{\textit{B) Effect of thresholding}}  \\
    %without threshold:
    w/o thresholding & 76.71 & 82.74 & 83.12 & 94.96 \\
    %DINOv2 B/14 & 76.71 & 82.74 & 83.12 & 94.96 \\
    %DINOv2 L/14 & 73.91 & 79.29 & 83.71 & 96.99 \\
    %with threshold:
    w/ thresholding & \textbf{16.58} & \textbf{24.07} & \textbf{25.99} & \textbf{38.42} \\
    %DINOv2 B/14 & 16.58 & 24.07 & \textbf{25.99} & \textbf{38.42} \\
    %DINOv2 L/14 & \textbf{15.51} & \textbf{23.38} & 27.3 & 43.22 \\
    \midrule
    \rowcolor{lightgray}
    \multicolumn{5}{l}{\textit{D) Effect of changing the resolution}}  \\
    %resolution 1x
    Resolution 1x & \textbf{12.41} & \textbf{18.63} & 29.38 & 37.73 \\
    %DINOv2 B/14 & 12.41 & 18.63 & 29.38 & 37.73 \\
    %DINOv2 L/14 & 11.32 & 16.23 & 30.65 & 39.19 \\
    %resolution 2x
    Resolution 2x & 12.73 & 19.49 & \textbf{24.78} & \textbf{34.03} \\
    %DINOv2 B/14 & 12.73 & 19.49 & 24.78 & 34.03 \\
    %DINOv2 L/14 & 11.72 & 18.14 & 25.46 & 35.83 \\
    %resolution 4x
    Resolution 4x & 16.58 & 24.07 & 25.99 & 38.42 \\
    %DINOv2 B/14 & 16.58 & 24.07 & \textbf{25.99} & \textbf{38.42} \\
    %DINOv2 L/14 & \textbf{15.51} & \textbf{23.38} & 27.3 & 43.22 \\
    \midrule
    \rowcolor{lightgray}
    \multicolumn{5}{l}{\textit{D) Effect of changing the backbone}}  \\
CLIP B/16 & 133.98 & 149.77 & 157.04 & 178.62 \\
CLIP L/14 & 120.81 & 142.62 & 131.36 & 155.96 \\
\hdashline
MAE B/16 & 112.47 & 128.08 & 146.86 & 170.48 \\
MAE L/16 & 129.09 & 142.19 & 159.01 & 182.23 \\
\hdashline
DINO ResNet50 & 64.84 & 78.07 & 81.72 & 103.26 \\
DINO ViT S/8 & 142.04 & 160.92 & 102.04 & 142.06 \\
DINO ViT B/8 & 43.29 & 61.69 & 42.23 & 59.36 \\
\hdashline
DINOv2 S/14 & 19.18 & 26.88 & 27.73 & 40.68 \\
DINOv2 B/14 & 16.58 & 24.07 & \textbf{25.99} & \textbf{38.42} \\
DINOv2 L/14 & \textbf{15.51} & \textbf{23.38} & 27.3 & 43.22 \\
DINOv2 S/14 reg. & 18.02 & 24.84 & 29.23 & 45.88 \\
DINOv2 B/14 reg. & 23.63 & 32.9 & 30.8 & 46.81 \\
DINOv2 L/14 reg. & 19.34 & 28.43 & 30.39 & 48.96 \\
\bottomrule
    \end{tabularx}
\end{adjustbox}
    \caption{\textbf{Ablation study on CARPK.} Impact of various components in our method. %: Sections \textit{A–C} assess individual processing choices, \textit{D} compares visual backbones, and \textit{E} evaluates the effect of exemplar count. 
    Unless specified otherwise, experiments use the DINOv2 ViT B/14 backbone.}

    \label{tab:carpk_ablation_vitb14}
\end{table*}

==> sec/XX_qualitatives_FSC_0_unfiltered.tex <==

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\figimg}[1]{\includegraphics[width=\figw, height=2.5cm]{#1}}
\arrayrulecolor{gray}

\begin{figure*}[t]
    \centering
    \tiny
    \newcommand{\hd}[1]{\textbf{#1}}
    \newcommand{\figw}{.26\textwidth}
    \setlength{\tabcolsep}{1pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{*6{C{\figw}}} %\begin{tabular}{r>{\hspace{0.1cm}}*6{p{\figw}>{\hspace{2pt}}}}

        % Row 1
        \large
        \figimg{images/supplementary/FSC/images/5918.jpg} &
        \figimg{images/supplementary/FSC/images/2207.jpg} &
        \figimg{images/supplementary/FSC/images/5574.jpg} &
        \figimg{images/supplementary/FSC/images/5934.jpg} &
        \figimg{images/supplementary/FSC/images/7714.jpg} &
        \figimg{images/supplementary/FSC/images/7573.jpg} \\
        \rowcolor[gray]{.9}
        12 &
        10 &
        90 &
        17 &
        45 &
        18 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5918.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5918.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2207.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2207.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5574.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5574.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5934.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5934.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7714.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7714.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7573.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7573.jpg} 
 \\
        12.0 &
        9.5 &
        90.9 &
        17.0 &
        49.8 &
        17.6 \\
        \arrayrulecolor{gray}
        \midrule

        % Row 2
        \large
        \figimg{images/supplementary/FSC/images/909.jpg} &
        \figimg{images/supplementary/FSC/images/340.jpg} &
        \figimg{images/supplementary/FSC/images/3341.jpg} &
        \figimg{images/supplementary/FSC/images/2053.jpg} &
        \figimg{images/supplementary/FSC/images/7341.jpg} &
        \figimg{images/supplementary/FSC/images/2239.jpg} \\
        \rowcolor[gray]{.9}
        62 &
        14 &
        35 &
        47 &
        17 &
        17 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/909.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/909.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/340.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/340.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/3341.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/3341.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2053.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2053.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7341.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7341.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2239.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2239.jpg} 
 \\
        61.8 &
        14.3 &
        40.2 &
        46.6 &
        17.1 &
        17.4 \\
        \midrule
        % Row 3
        \large
        \figimg{images/supplementary/FSC/images/5360.jpg} &
        \figimg{images/supplementary/FSC/images/5562.jpg} &
        \figimg{images/supplementary/FSC/images/5797.jpg} &
        \figimg{images/supplementary/FSC/images/6251.jpg} &
        \figimg{images/supplementary/FSC/images/2932.jpg} &
        \figimg{images/supplementary/FSC/images/301.jpg} \\
        \rowcolor[gray]{.9}
        65 &
        13 &
        58 &
        25 &
        24 &
        28 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5360.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5360.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5562.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5562.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5797.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5797.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/6251.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/6251.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2932.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2932.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/301.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/301.jpg} 
 \\
        66.5 &
        13.2 &
        57.8 &
        24.5 &
        24.5 &
        27.7 \\

        % Row 4
        \large
        \figimg{images/supplementary/FSC/images/2189.jpg} &
        \figimg{images/supplementary/FSC/images/5916.jpg} &
        \figimg{images/supplementary/FSC/images/6928.jpg} &
        \figimg{images/supplementary/FSC/images/4073.jpg} &
        \figimg{images/supplementary/FSC/images/5600.jpg} &
        \figimg{images/supplementary/FSC/images/7713.jpg} \\
        \rowcolor[gray]{.9}
        8 &
        38 &
        29 &
        25 &
        149 &
        19 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2189.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2189.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5916.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5916.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/6928.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/6928.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/4073.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/4073.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5600.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5600.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7713.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7713.jpg} 
 \\
        7.8 &
        37.2 &
        29.5 &
        27.5 &
        151.5 &
        19.5 \\

        % Row 5
        \large
        \figimg{images/supplementary/FSC/images/2029.jpg} &
        \figimg{images/supplementary/FSC/images/7295.jpg} &
        \figimg{images/supplementary/FSC/images/5363.jpg} &
        \figimg{images/supplementary/FSC/images/2019.jpg} &
        \figimg{images/supplementary/FSC/images/4500.jpg} &
        \figimg{images/supplementary/FSC/images/7173.jpg} \\
        \rowcolor[gray]{.9}
        78 &
        63 &
        34 &
        14 &
        7 &
        47 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2029.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2029.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7295.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7295.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5363.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5363.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2019.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2019.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/4500.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/4500.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7173.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7173.jpg} 
 \\
        78.6 &
        60.6 &
        35.0 &
        14.9 &
        8.6 &
        51.8 \\


    \end{tabular}
    }
    \caption{\textbf{Qualitative results.}}
    \label{fig:more-examples-0}
\end{figure*}


==> sec/XX_qualitatives_FSC_1_unfiltered.tex <==

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\figimg}[1]{\includegraphics[width=\figw, height=2.5cm]{#1}}


\begin{figure*}[t]
    \centering
    \tiny
    \newcommand{\hd}[1]{\textbf{#1}}
    \newcommand{\figw}{.26\textwidth}
    \setlength{\tabcolsep}{1pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{*6{C{\figw}}} %\begin{tabular}{r>{\hspace{0.1cm}}*6{p{\figw}>{\hspace{2pt}}}}

        % Row 6
        \large
        \figimg{images/supplementary/FSC/images/2209.jpg} &
        \figimg{images/supplementary/FSC/images/3655.jpg} &
        \figimg{images/supplementary/FSC/images/4919.jpg} &
        \figimg{images/supplementary/FSC/images/2179.jpg} &
        \figimg{images/supplementary/FSC/images/7683.jpg} &
        \figimg{images/supplementary/FSC/images/6892.jpg} \\
        \rowcolor[gray]{.9}
        11 &
        13 &
        30 &
        15 &
        34 &
        54 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2209.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2209.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/3655.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/3655.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/4919.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/4919.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2179.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2179.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7683.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7683.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/6892.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/6892.jpg} 
 \\
        11.4 &
        13.9 &
        30.7 &
        16.7 &
        39.6 &
        55.0 \\

        % Row 7
        \large
        \figimg{images/supplementary/FSC/images/3645.jpg} &
        \figimg{images/supplementary/FSC/images/2155.jpg} &
        \figimg{images/supplementary/FSC/images/7401.jpg} &
        \figimg{images/supplementary/FSC/images/4928.jpg} &
        \figimg{images/supplementary/FSC/images/7174.jpg} &
        \figimg{images/supplementary/FSC/images/1572.jpg} \\
        \rowcolor[gray]{.9}
        59 &
        18 &
        90 &
        39 &
        96 &
        25 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/3645.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/3645.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2155.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2155.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7401.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7401.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/4928.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/4928.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7174.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7174.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/1572.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/1572.jpg} 
 \\
        60.0 &
        17.8 &
        89.8 &
        39.2 &
        94.4 &
        27.2 \\

        % Row 8
        \large
        \figimg{images/supplementary/FSC/images/7389.jpg} &
        \figimg{images/supplementary/FSC/images/5818.jpg} &
        \figimg{images/supplementary/FSC/images/5823.jpg} &
        \figimg{images/supplementary/FSC/images/5357.jpg} &
        \figimg{images/supplementary/FSC/images/7283.jpg} &
        \figimg{images/supplementary/FSC/images/2270.jpg} \\
        \rowcolor[gray]{.9}
        24 &
        55 &
        69 &
        12 &
        22 &
        50 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7389.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7389.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5818.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5818.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5823.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5823.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5357.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5357.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7283.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7283.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2270.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2270.jpg} 
 \\
        25.2 &
        57.3 &
        67.4 &
        12.6 &
        22.3 &
        51.5 \\

        % Row 9
        \large
        \figimg{images/supplementary/FSC/images/348.jpg} &
        \figimg{images/supplementary/FSC/images/2910.jpg} &
        \figimg{images/supplementary/FSC/images/3696.jpg} &
        \figimg{images/supplementary/FSC/images/7134.jpg} &
        \figimg{images/supplementary/FSC/images/7605.jpg} &
        \figimg{images/supplementary/FSC/images/7136.jpg} \\
        \rowcolor[gray]{.9}
        27 &
        14 &
        7 &
        22 &
        20 &
        87 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/348.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/348.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2910.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2910.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/3696.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/3696.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7134.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7134.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7605.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7605.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7136.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7136.jpg} 
 \\
        25.4 &
        15.0 &
        7.5 &
        21.6 &
        19.3 &
        84.9 \\

        % Row 10
        \large
        \figimg{images/supplementary/FSC/images/6247.jpg} &
        \figimg{images/supplementary/FSC/images/7096.jpg} &
        \figimg{images/supplementary/FSC/images/2947.jpg} &
        \figimg{images/supplementary/FSC/images/307.jpg} &
        \figimg{images/supplementary/FSC/images/5362.jpg} &
        \figimg{images/supplementary/FSC/images/5830.jpg} \\
        \rowcolor[gray]{.9}
        15 &
        19 &
        35 &
        21 &
        18 &
        35 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/6247.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/6247.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7096.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7096.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2947.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2947.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/307.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/307.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5362.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5362.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5830.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5830.jpg} 
 \\
        14.2 &
        19.9 &
        34.0 &
        21.6 &
        17.9 &
        33.9 \\

        % Row 11
        \large
        \figimg{images/supplementary/FSC/images/2163.jpg} &
        \figimg{images/supplementary/FSC/images/2141.jpg} &
        \figimg{images/supplementary/FSC/images/708.jpg} &
        \figimg{images/supplementary/FSC/images/4116.jpg} &
        \figimg{images/supplementary/FSC/images/5921.jpg} &
        \figimg{images/supplementary/FSC/images/2617.jpg} \\
        \rowcolor[gray]{.9}
        13 &
        11 &
        14 &
        14 &
        30 &
        41 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2163.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2163.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2141.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2141.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/708.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/708.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/4116.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/4116.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5921.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5921.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2617.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2617.jpg} 
 \\
        13.6 &
        11.9 &
        14.0 &
        15.5 &
        31.4 &
        38.7 \\


    \end{tabular}
    }
    \caption{\textbf{Qualitative results.}}
    \label{fig:more-examples-1}
\end{figure*}


==> sec/XX_qualitatives_FSC_2_unfiltered.tex <==

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\figimg}[1]{\includegraphics[width=\figw, height=2.5cm]{#1}}


\begin{figure*}[t]
    \centering
    \tiny
    \newcommand{\hd}[1]{\textbf{#1}}
    \newcommand{\figw}{.26\textwidth}
    \setlength{\tabcolsep}{1pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{*6{C{\figw}}} %\begin{tabular}{r>{\hspace{0.1cm}}*6{p{\figw}>{\hspace{2pt}}}}

        % Row 12
        \large
        \figimg{images/supplementary/FSC/images/6268.jpg} &
        \figimg{images/supplementary/FSC/images/4496.jpg} &
        \figimg{images/supplementary/FSC/images/5512.jpg} &
        \figimg{images/supplementary/FSC/images/4916.jpg} &
        \figimg{images/supplementary/FSC/images/5944.jpg} &
        \figimg{images/supplementary/FSC/images/6771.jpg} \\
        \rowcolor[gray]{.9}
        24 &
        13 &
        72 &
        91 &
        15 &
        24 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/6268.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/6268.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/4496.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/4496.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5512.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5512.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/4916.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/4916.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5944.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5944.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/6771.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/6771.jpg} 
 \\
        26.7 &
        14.1 &
        70.9 &
        91.7 &
        14.0 &
        24.4 \\

        % Row 13
        \large
        \figimg{images/supplementary/FSC/images/6650.jpg} &
        \figimg{images/supplementary/FSC/images/5836.jpg} &
        \figimg{images/supplementary/FSC/images/7263.jpg} &
        \figimg{images/supplementary/FSC/images/7682.jpg} &
        \figimg{images/supplementary/FSC/images/7536.jpg} &
        \figimg{images/supplementary/FSC/images/4932.jpg} \\
        \rowcolor[gray]{.9}
        20 &
        18 &
        42 &
        24 &
        24 &
        56 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/6650.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/6650.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5836.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5836.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7263.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7263.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7682.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7682.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7536.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7536.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/4932.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/4932.jpg} 
 \\
        18.8 &
        17.0 &
        44.7 &
        22.5 &
        23.9 &
        55.5 \\

        % Row 14
        \large
        \figimg{images/supplementary/FSC/images/6810.jpg} &
        \figimg{images/supplementary/FSC/images/4883.jpg} &
        \figimg{images/supplementary/FSC/images/290.jpg} &
        \figimg{images/supplementary/FSC/images/3697.jpg} &
        \figimg{images/supplementary/FSC/images/4939.jpg} &
        \figimg{images/supplementary/FSC/images/7118.jpg} \\
        \rowcolor[gray]{.9}
        39 &
        15 &
        12 &
        11 &
        20 &
        33 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/6810.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/6810.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/4883.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/4883.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/290.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/290.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/3697.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/3697.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/4939.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/4939.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7118.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7118.jpg} 
 \\
        40.4 &
        16.1 &
        13.7 &
        10.3 &
        21.1 &
        34.1 \\

        % Row 15
        \large
        \figimg{images/supplementary/FSC/images/6659.jpg} &
        \figimg{images/supplementary/FSC/images/5841.jpg} &
        \figimg{images/supplementary/FSC/images/7586.jpg} &
        \figimg{images/supplementary/FSC/images/4079.jpg} &
        \figimg{images/supplementary/FSC/images/287.jpg} &
        \figimg{images/supplementary/FSC/images/6053.jpg} \\
        \rowcolor[gray]{.9}
        8 &
        51 &
        35 &
        24 &
        21 &
        108 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/6659.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/6659.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/5841.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/5841.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7586.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7586.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/4079.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/4079.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/287.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/287.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/6053.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/6053.jpg} 
 \\
        10.3 &
        50.8 &
        33.4 &
        26.9 &
        21.8 &
        106.3 \\

        % Row 16
        \large
        \figimg{images/supplementary/FSC/images/293.jpg} &
        \figimg{images/supplementary/FSC/images/4967.jpg} &
        \figimg{images/supplementary/FSC/images/713.jpg} &
        \figimg{images/supplementary/FSC/images/2931.jpg} &
        \figimg{images/supplementary/FSC/images/6960.jpg} &
        \figimg{images/supplementary/FSC/images/2045.jpg} \\
        \rowcolor[gray]{.9}
        41 &
        19 &
        24 &
        43 &
        19 &
        21 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/293.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/293.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/4967.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/4967.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/713.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/713.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2931.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2931.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/6960.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/6960.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2045.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2045.jpg} 
 \\
        42.1 &
        17.9 &
        22.6 &
        39.2 &
        19.8 &
        23.8 \\

        % Row 17
        \large
        \figimg{images/supplementary/FSC/images/4879.jpg} &
        \figimg{images/supplementary/FSC/images/7216.jpg} &
        \figimg{images/supplementary/FSC/images/2262.jpg} &
        \figimg{images/supplementary/FSC/images/1884.jpg} \\
        \rowcolor[gray]{.9}
        75 &
        24 &
        9 &
        16 \\
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/4879.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/4879.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/7216.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/7216.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/2262.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/2262.jpg} 
 &
        \includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps_no_bkg_threshold/1884.jpg}\includegraphics[width=0.45\linewidth, height=1.5cm]{images/supplementary/FSC/densitymaps/1884.jpg} 
 \\
        76.1 &
        26.3 &
        7.6 &
        17.1 \\


    \end{tabular}
    }
    \caption{\textbf{Qualitative results.}}
    \label{fig:more-examples-2}
\end{figure*}


==> sec/table_carpk.tex <==
\begin{table}[!ht]
    \caption{\textbf{Results on the CARPK dataset~\cite{DBLP:conf/iccv/HsiehLH17}.} We report the performance in terms of MAE and RMSE obtained with some of the methodologies discussed in this survey over the CARPK benchmark. Following previous literature, CARPK is exploited for testing cross-dataset generalization over a specific object class -- vehicles. The best results are in bold. }
    \label{tab:carpk_results}
    \setlength{\tabcolsep}{2pt}
    \footnotesize
    \newcolumntype{C}{>{\centering\arraybackslash}m{.19\linewidth}}
    \newcolumntype{Z}{>{\centering\arraybackslash}m{.14\linewidth}}
    \center
    \begin{tabularx}{0.99\linewidth}{lCZZ}
            \toprule
            Method & Fine-Tuned & \textit{MAE} $\downarrow$ & \textit{RMSE} $\downarrow$ \\
            \midrule
            \midrule
            \textit{Baseline} & & & \\
            Mean & N/A & 65.63 & 72.26 \\
            Median & N/A & 67.88 & 74.58 \\
            \midrule
            \textit{Reference-based (12 exemplars)} & & & \\
            %GMN$^*$~\cite{DBLP:conf/accv/LuXZ18} & \cmark & 7.48 & 9.90 \\
            FamNet~\cite{DBLP:conf/cvpr/RanjanSNH21} & \cmark & 18.19 & 33.66 \\
            % CFOCNet~\cite{DBLP:conf/wacv/YangSHC21} & - & - & - \\
            % VCN~\cite{DBLP:conf/cvpr/RanjanH22} & - & - & - \\
            RCAC~\cite{DBLP:conf/eccv/GongZ0DS22} & \cmark & 13.62 & 19.08 \\
            % MACnet~\cite{DBLP:journals/prl/McCarthyVOTAH23} & - & - & - \\
            BMNet+~\cite{DBLP:conf/cvpr/Shi0FL022} & \cmark & 5.76 & 7.83 \\
            SPDCN~\cite{DBLP:conf/bmvc/LinYM0LLHYC22} & \cmark & 10.07 & 14.12 \\
            SAFECount~\cite{DBLP:conf/wacv/YouYLLCL23} & \cmark & 5.33 & 7.04 \\
            CSTrans~\cite{DBLP:journals/pr/GaoH24} & \cmark & 5.06 & 6.53 \\
            CountVers~\cite{DBLP:journals/kbs/YangCDWZ24} & \cmark & 5.19 & 6.55 \\
            CACViT~\cite{DBLP:conf/aaai/WangX0024} & \cmark & \textbf{4.91} & \textbf{6.49} \\
            %CFENet~\cite{DBLP:journals/ivc/ZhangZCWH25} & \cmark & \textbf{4.56} & \textbf{5.74} \\
            %MEAMNet~\cite{DBLP:journals/prl/ZhangHZLCL24} & \cmark & 4.93 & 6.50 \\
            \noalign{\vskip 2pt} 
            \hdashline
            \noalign{\vskip 2pt}
            FamNet~\cite{DBLP:conf/cvpr/RanjanSNH21} & \xmark & 28.84 & 44.47 \\
            RCAC~\cite{DBLP:conf/eccv/GongZ0DS22} & \xmark & 17.98 & 24.21 \\
            BMNet+~\cite{DBLP:conf/cvpr/Shi0FL022} & \xmark & 10.44 & 13.77 \\
            SPDCN~\cite{DBLP:conf/bmvc/LinYM0LLHYC22} & \xmark & 18.15 & 21.61 \\
            ConCoNet (FamNet)~\cite{DBLP:journals/prl/SolivenVOTAH23} & \xmark & 23.55 & 32.41 \\
            ConCoNet (BMNet)~\cite{DBLP:journals/prl/SolivenVOTAH23} & \xmark & 16.40 & 21.54 \\
            %ASFNet~\cite{10145320} & - & - & - \\
            SAFECount~\cite{DBLP:conf/wacv/YouYLLCL23} & \xmark & 16.66 & 24.08 \\
            LOCA~\cite{DBLP:conf/iccv/EukicLZK23} & \xmark & 9.97 & 12.51 \\
            SATCount~\cite{DBLP:journals/nn/WangYWLC24} & \xmark & 9.51 & 12.67 \\
            CACViT~\cite{DBLP:conf/aaai/WangX0024} & \xmark & 8.30 & 11.18 \\
            SSD~\cite{DBLP:conf/ijcai/Xu0Z24} & \xmark & 9.58 & 12.15 \\
            % DAVE~\cite{DBLP:conf/cvpr/PelhanLZK24} & - & - & - \\ 
            TFPOC~\cite{DBLP:conf/wacv/Shi0Z24} & \xmark & 10.97 & 14.24 \\
            UPC~\cite{DBLP:conf/aaai/0018C24} & \xmark & \textbf{7.83} & \textbf{9.74} \\
            %CFENet~\cite{DBLP:journals/ivc/ZhangZCWH25} & \xmark & 10.68 & 13.25 \\
            % CAP~\cite{10671540} & \xmark & 9.11 & 11.02 \\
            %\midrule
            %\textit{Reference-less} & & & \\
            % RepRPN-Counter~\cite{DBLP:conf/accv/RanjanN22} & - & - & - \\
            %RCC~\cite{DBLP:journals/corr/abs-2205-10203} & \cmark & 9.21 & 11.33 \\
            %RCC~\cite{DBLP:journals/corr/abs-2205-10203} & \xmark & 12.31 & 15.40 \\
            %CounTR~\cite{DBLP:conf/bmvc/LiuZZX22} & \cmark & 5.75 & 7.45 \\
            % GCNet~\cite{DBLP:journals/pr/WangLZTG24} & - & - & - \\ 
            \midrule
            \textit{Open-world Text-guided} & & & \\
            % ZSC~\cite{DBLP:conf/cvpr/XuL0RS23} & - & - & - \\
            %CounTX~\cite{AminiNaieni23} & \cmark & 8.13 & 10.87 \\
            CounTX~\cite{AminiNaieni23} & \xmark & 11.64 & 14.85 \\ 
            CLIP-Count~\cite{DBLP:conf/mm/JiangLC23} & \xmark & 11.96 & 16.61 \\
            VLCounter~\cite{DBLP:conf/aaai/KangMKH24} & \xmark & \textbf{6.46} & \textbf{8.68} \\
            VA-Count~\cite{DBLP:conf/eccv/ZhuYYGWZH24} & \xmark & 10.63 & 13.20 \\
            TFPOC$^{\ddagger}$~\cite{DBLP:conf/wacv/Shi0Z24} & \xmark & 11.01 & 14.34 \\
            UPC~\cite{DBLP:conf/aaai/0018C24}$^{\ddagger}$ & \xmark & 7.62 & 9.71 \\
            % CountGD~\cite{DBLP:journals/corr/abs-2407-04619} & \xmark & 3.68 & 5.17 \\
            \bottomrule \\
    \end{tabularx}

     {\setlength{\baselineskip}{0.7\baselineskip}\footnotesize
    %* GMN uses extra training data from the ILSVRC video dataset~\cite{DBLP:journals/ijcv/RussakovskyDSKS15}, which consists of video sequences of cars; 
    $\ddagger$ prompt-based modification of a reference-based method.}
\end{table}
